Model comparison of the transverse momentum spectra of charged hadrons produced in $PbPb$ collision at $\sqrt{s_{NN}} = 5.02$ TeV

Transverse Momentum, $p_T$, spectra is of prime importance in order to extract crucial information about the evolution dynamics of the system of particles produced in the collider experiments. In this work, the transverse momentum spectra of charged hadrons produced in $PbPb$ collision at $5.02$ TeV has been analyzed using different distribution functions in order to gain strong insight into the information that can be extracted from the spectra. We have also discussed the applicability of Pearson distribution on the spectra of charged hadron at $5.02$ TeV.

==> ref.tex <==
 
 \begin{thebibliography}{9}
 %REF 1
  \bibitem{RHIC_exp}
 M. Harrison, T. Ludlam, S. Ozaki,
\textit{RHIC project overview}, Nucl. Instrum. Methods Phys. Res. A 499 (2) (2003) 235–244

%REF 2
%\cite{Evans:2008zzb}
\bibitem{Evans:2008zzb}
L.~Evans and P.~Bryant,
\textit{LHC Machine},
JINST \textbf{3}, S08001 (2008)
%doi:10.1088/1748-0221/3/08/S08001
%3183 citations counted in INSPIRE as of 18 Oct 2020

 
%REF 3
%\cite{Jacobs:2004qv}
\bibitem{Jacobs:2004qv} 
  P.~Jacobs and X.~N.~Wang,
  \textit{ Matter in extremis: Ultrarelativistic nuclear collisions at RHIC},
  Prog.\ Part.\ Nucl.\ Phys.\  {\bf 54}, 443 (2005)
%  doi:10.1016/j.ppnp.2004.09.001
  [hep-ph/0405125].
  %%CITATION = doi:10.1016/j.ppnp.2004.09.001;%%
  %247 citations counted in INSPIRE as of 03 Jan 2020
 
%REF 4  
  %\cite{Gyulassy:2003mc}
\bibitem{Gyulassy:2003mc} 
  M.~Gyulassy, I.~Vitev, X.~N.~Wang and B.~W.~Zhang,
  \textit{Jet quenching and radiative energy loss in dense nuclear matter},
  In *Hwa, R.C. (ed.) et al.: Quark gluon plasma* 123-191 %doi:10.1142/9789812795533\_0003
  [nucl-th/0302077].
  %%CITATION = doi:10.1142/9789812795533_0003;%%
  %492 citations counted in INSPIRE as of 03 Jan 2020

%REF 5
%\cite{Kolb:2003dz}
\bibitem{Kolb:2003dz} 
  P.~F.~Kolb and U.~W.~Heinz,
  \textit{Hydrodynamic description of ultrarelativistic heavy ion collisions},
  In *Hwa, R.C. (ed.) et al.: Quark gluon plasma* 634-714
  [nucl-th/0305084].
  %%CITATION = NUCL-TH/0305084;%%
  %844 citations counted in INSPIRE as of 03 Jan 2020

%REF 6
%\cite{Jena:2020wno}
\bibitem{Jena:2020wno}
S.~Jena and R.~Gupta,
\textit{A unified formalism to study transverse momentum spectra in heavy-ion collision},
Phys. Lett. B \textbf{807}, 135551 (2020)
%doi:10.1016/j.physletb.2020.135551
%0 citations counted in INSPIRE as of 03 Oct 2020

%REF 7
     \bibitem{Koppe:1948}
  H.~Koppe,
  Z. Naturforschg. {\bf 3 a}, 251-252 (1948).

%REF 8  
  %\cite{Tawfik:2013tza}
\bibitem{Tawfik:2013tza} 
  A.~N.~Tawfik,
  \textit{Koppe's Work of 1948: A fundamental for non-equilibrium rate of particle production},
  Z. Naturforsch. A {\bf 69}, 106 (2014)
%  doi:10.5560/ZNA.2013-0077
 % [arXiv:1312.1968 [nucl-th]].
  %%CITATION = doi:10.5560/ZNA.2013-0077;%%
  %3 citations counted in INSPIRE as of 07 Jan 2020
  
%REF 9  
  \bibitem{fermi:ptp}
  E.~Fermi,
  \textit{High-energy nuclear events},
  Prog. Theor. Phys. {\bf 5}, 570 (1950)
  
%REF 10  
  %\cite{Fermi:1951zz}
\bibitem{Fermi:1951zz} 
  E.~Fermi,
  \textit{Angular Distribution of the Pions Produced in High Energy Nuclear Collisions},
  Phys. Rev. {\bf 81}, 683 (1951).
%  doi:10.1103/PhysRev.81.683
  %%CITATION = doi:10.1103/PhysRev.81.683;%%
  %149 citations counted in INSPIRE as of 07 Jan 2020

%REF 11 
 %\cite{Hagedorn:1965st}
\bibitem{Hagedorn:1965st} 
  R.~Hagedorn,
  \textit{Statistical thermodynamics of strong interactions at high-energies},
  Nuovo Cim.\ Suppl.\  {\bf 3}, 147 (1965).
  %%CITATION = NUCUA,3,147;%%
  %1583 citations counted in INSPIRE as of 07 Jan 2020
 
 %REF 12
   %\cite{Hagedorn:1967ua}
\bibitem{Hagedorn:1967ua} 
  R.~Hagedorn and J.~Ranft,
  \textit{Statistical thermodynamics of strong interactions at high-energies. 2. Momentum spectra of particles produced in pp-collisions},
  Nuovo Cim.\ Suppl.\  {\bf 6}, 169 (1968).
  %%CITATION = NUCUA,6,169;%%
  %330 citations counted in INSPIRE as of 03 Jan 2020

%REF 13
  %\cite{Tawfik:2014eba}
\bibitem{Tawfik:2014eba}
A.~N.~Tawfik,
\textit{Equilibrium statistical-thermal models in high-energy physics},
Int. J. Mod. Phys. A \textbf{29}, no.17, 1430021 (2014)
% doi:10.1142/S0217751X1430021X
[arXiv:1410.0372 [hep-ph]].
%47 citations counted in INSPIRE as of 23 Sep 2020

%REF 14
%\cite{DeGroot:1980dk}
\bibitem{DeGroot:1980dk} 
  S.~R.~De Groot, W.~A.~Van Leeuwen and C.~G.~Van Weert,
  \textit{Relativistic Kinetic Theory. Principles and Applications},
  Amsterdam, Netherlands: North-holland ( 1980) 417p
  %78 citations counted in INSPIRE as of 03 Jan 2020

%REF 15  
  %\cite{Stodolsky:1995ds}
\bibitem{Stodolsky:1995ds}
L.~Stodolsky,
\textit{Temperature fluctuations in multiparticle production},
Phys. Rev. Lett. \textbf{75}, 1044-1045 (1995)
% doi:10.1103/PhysRevLett.75.1044
%156 citations counted in INSPIRE as of 23 Sep 2020

%REF 16
  %\cite{Schnedermann:1993ws}
\bibitem{Schnedermann:1993ws}
E.~Schnedermann, J.~Sollfrank and U.~W.~Heinz,
\textit{Thermal phenomenology of hadrons from 200-A/GeV S+S collisions},
Phys. Rev. C \textbf{48}, 2462-2475 (1993)
% doi:10.1103/PhysRevC.48.2462
[arXiv:nucl-th/9307020 [nucl-th]].
%948 citations counted in INSPIRE as of 23 Sep 2020

%REF 17
%\cite{Basu:2015zra}
\bibitem{Basu:2015zra}
S.~Basu, R.~Chatterjee, B.~K.~Nandi and T.~K.~Nayak,
\textit{Characterization of relativistic heavy-ion collisions at the Large Hadron Collider through temperature fluctuations},
[arXiv:1504.04502 [nucl-ex]].
%5 citations counted in INSPIRE as of 23 Sep 2020

%REF 18  
  %\cite{Pulawski:2017sct}
\bibitem{Pulawski:2017sct}
S.~Pulawski,
\textit{Recent results from the strong interactions program of NA61/SHINE},
EPJ Web Conf. \textbf{164}, 07033 (2017)
% doi:10.1051/epjconf/201716407033
[arXiv:1705.02462 [nucl-ex]].
%1 citations counted in INSPIRE as of 23 Sep 2020
  
   %REF 19
  %\cite{Tsallis:1987eu}
\bibitem{Tsallis:1987eu} 
  C.~Tsallis,
  \textit{Possible Generalization of Boltzmann-Gibbs Statistics},
  J.\ Statist.\ Phys.\  {\bf 52}, 479 (1988).
%  doi:10.1007/BF01016429
  %%CITATION = doi:10.1007/BF01016429;%%
  %1103 citations counted in INSPIRE as of 03 Jan 2020
  
%REF 20  
  %\cite{Wilk:1999dr}
\bibitem{Wilk:1999dr} 
  G.~Wilk and Z.~Wlodarczyk,
  \textit{On the interpretation of nonextensive parameter q in Tsallis statistics and Levy distributions},
  Phys.\ Rev.\ Lett.\  {\bf 84}, 2770 (2000)
 % doi:10.1103/PhysRevLett.84.2770
  [hep-ph/9908459].
  %%CITATION = doi:10.1103/PhysRevLett.84.2770;%%
  %249 citations counted in INSPIRE as of 03 Jan 2020
 
 %REF 21 
  %\cite{Wilk:2012zn}
\bibitem{Wilk:2012zn} 
  G.~Wilk and Z.~Wlodarczyk,
  \textit{Consequences of temperature fluctuations in observables measured in high energy collisions},
  Eur.\ Phys.\ J.\ A {\bf 48}, 161 (2012)
%  doi:10.1140/epja/i2012-12161-y
  [arXiv:1203.4452 [hep-ph]].
  %%CITATION = doi:10.1140/epja/i2012-12161-y;%%
  %47 citations counted in INSPIRE as of 03 Jan 2020
 


%REF 22  
  \bibitem{tsallisbook}
  C.~Tsallis,
  Introduction to Nonextensive Statistical Mechanics (Springer, 2009)

%REF 23  
  \bibitem{tsallisgellmannbook}
  M. Gell-Mann and C. Tsallis, 
  Nonextensive Entropy-Interdisciplinary Application (Oxford University Press, 2004).

%REF 24
%\cite{Cleymans:2012ya}
\bibitem{Cleymans:2012ya} 
  J.~Cleymans and D.~Worku,
  \textit{Relativistic Thermodynamics: Transverse Momentum Distributions in High-Energy Physics},
  Eur.\ Phys.\ J.\ A {\bf 48}, 160 (2012)
%  doi:10.1140/epja/i2012-12160-0
  [arXiv:1203.4343 [hep-ph]].
  %%CITATION = doi:10.1140/epja/i2012-12160-0;%%
  %125 citations counted in INSPIRE as of 03 Jan 2020
%REF 25
 %\cite{Biro:2011bq}
\bibitem{Biro:2011bq} 
  T.~S.~Biro and E.~Molnar,
  \textit{Fluid dynamical equations and transport coefficients of relativistic gases with non-extensive statistics},
  Phys.\ Rev.\ C {\bf 85}, 024905 (2012)
 % doi:10.1103/PhysRevC.85.024905
  [arXiv:1109.2482 [nucl-th]].
  %%CITATION = doi:10.1103/PhysRevC.85.024905;%%
  %15 citations counted in INSPIRE as of 03 Jan 2020
  
 %REF 26 
  %\cite{Wilk:2000yv}
\bibitem{Wilk:2000yv} 
  G.~Wilk and Z.~Wlodarczyk,
  \textit{The Imprints of nonextensive statistical mechanics in high-energy collisions},
  Chaos Solitons Fractals {\bf 13}, 581 (2002)
 % doi:10.1016/S0960-0779(01)00041-8
  [hep-ph/0004250].
  %%CITATION = doi:10.1016/S0960-0779(01)00041-8;%%
  %44 citations counted in INSPIRE as of 03 Jan 2020
 
 %REF 27
 %\cite{Wilk:2008ue}
\bibitem{Wilk:2008ue} 
  G.~Wilk and Z.~Wlodarczyk,
  \textit{Power laws in elementary and heavy-ion collisions: A Story of fluctuations and nonextensivity?},
  Eur.\ Phys.\ J.\ A {\bf 40}, 299 (2009)
 % doi:10.1140/epja/i2009-10803-9
  [arXiv:0810.2939 [hep-ph]].
  %%CITATION = doi:10.1140/epja/i2009-10803-9;%%
  %139 citations counted in INSPIRE as of 03 Jan 2020

%REF 28
%\cite{Biro:2005uv}
\bibitem{Biro:2005uv} 
  T.~S.~Biro and G.~Purcsel,
  \textit{Non-extensive Boltzmann equation and hadronization},
  Phys.\ Rev.\ Lett.\  {\bf 95}, 162302 (2005)
 % doi:10.1103/PhysRevLett.95.162302
  [hep-ph/0503204].
  %%CITATION = doi:10.1103/PhysRevLett.95.162302;%%
  %58 citations counted in INSPIRE as of 03 Jan 2020 
  
 %REF 29 
  %\cite{Si:2017cyg}
\bibitem{Si:2017cyg} 
  R.~F.~Si, H.~L.~Li and F.~H.~Liu,
  \textit{Comparing standard distribution and its Tsallis form of transverse momenta in high energy collisions},
  Adv.\ High Energy Phys.\  {\bf 2018}, 7895967 (2018)
%  doi:10.1155/2018/7895967
  [arXiv:1710.09645 [nucl-th]].
  %%CITATION = doi:10.1155/2018/7895967;%%
  %4 citations counted in INSPIRE as of 03 Jan 2020

%REF 30  
  %\cite{De:2007zza}
\bibitem{De:2007zza} 
  B.~De, S.~Bhattacharyya, G.~Sau and S.~K.~Biswas,
  \textit{Non-extensive thermodynamics, heavy ion collisions and particle production at RHIC energies},
  Int.\ J.\ Mod.\ Phys.\ E {\bf 16}, 1687 (2007).
%  doi:10.1142/S0218301307006976
  %%CITATION = doi:10.1142/S0218301307006976;%%
  %20 citations counted in INSPIRE as of 03 Jan 2020

%REF 31  
  %\cite{Arnison:1982ed}
\bibitem{Arnison:1982ed} 
  G.~Arnison {\it et al.} [UA1 Collaboration],
  \textit{Transverse Momentum Spectra for Charged Particles at the CERN Proton anti-Proton Collider},
  Phys.\ Lett.\  {\bf 118B}, 167 (1982).
%  doi:10.1016/0370-2693(82)90623-2
  %%CITATION = doi:10.1016/0370-2693(82)90623-2;%%
  %454 citations counted in INSPIRE as of 03 Jan 2020

%REF 32
%\cite{Wong:2012zr}
\bibitem{Wong:2012zr} 
  C.~Y.~Wong and G.~Wilk,
  \textit{Tsallis Fits to \pt~ Spectra for pp Collisions at LHC},
  Acta Phys.\ Polon.\ B {\bf 43}, 2047 (2012)
%  doi:10.5506/APhysPolB.43.2047
  [arXiv:1210.3661 [hep-ph]].
  %%CITATION = doi:10.5506/APhysPolB.43.2047;%%
  %56 citations counted in INSPIRE as of 03 Jan 2020

%REF 33
  %\cite{Biyajima:2016fpb}
\bibitem{Biyajima:2016fpb} 
  M.~Biyajima, T.~Mizoguchi and N.~Suzuki,
  \textit{Analyses of whole transverse momentum distributions in $p\bar{p}$ and $pp$ collisions by using a modified version of Hagedorn’s formula},
  Int.\ J.\ Mod.\ Phys.\ A {\bf 32}, no. 11, 1750057 (2017)
 % doi:10.1142/S0217751X17500579
  [arXiv:1604.01264 [hep-ph]].
  %%CITATION = doi:10.1142/S0217751X17500579;%%
  %17 citations counted in INSPIRE as of 03 Jan 2020

%REF 34
%\cite{Michael:1976pz}
\bibitem{Michael:1976pz} 
  C.~Michael and L.~Vanryckeghem,
  \textit{Consequences of Momentum Conservation for Particle Production at Large Transverse Momentum},
  J.\ Phys.\ G {\bf 3}, L151 (1977).
 % doi:10.1088/0305-4616/3/8/002
  %%CITATION = doi:10.1088/0305-4616/3/8/002;%%
  %35 citations counted in INSPIRE as of 03 Jan 2020

%REF 35
%\cite{Michael:1977hx}
\bibitem{Michael:1977hx} 
  C.~Michael,
  \textit{Large Transverse Momentum and Large Mass Production in Hadronic Interactions},
  Prog.\ Part.\ Nucl.\ Phys.\  {\bf 2}, 1 (1979).
 % doi:10.1016/0146-6410(79)90002-4
  %%CITATION = doi:10.1016/0146-6410(79)90002-4;%%
  %30 citations counted in INSPIRE as of 03 Jan 2020
  
%REF 36  
 \bibitem{Pearson343}
 K. Pearson, 
 Philosophical Transactions of the Royal Society of London A: Mathematical, Physical and Engineering Sciences 186, 343 (1895)
 
%REF 37
\bibitem{pollard}
J. H. Pollard, 
Numerical and Statistical Techniques (Cambridge University Press, 1979)
%REF 38
\bibitem{root}
 R. Brun and F. Rademakers 1997 ROOT - An Object Oriented Data Analysis Framework,Nucl. Instrum.Meth. A38981. See also ”ROOT [software], Release v6.08.06, doi:10.5281/zenodo.848819

%REF 39
%\cite{James:1975dr}
\bibitem{James:1975dr}
F.~James and M.~Roos,
\textit{Minuit: A System for Function Minimization and Analysis of the Parameter Errors and Correlations},
Comput. Phys. Commun. \textbf{10}, 343-367 (1975)
%doi:10.1016/0010-4655(75)90039-9
%2513 citations counted in INSPIRE as of 15 Oct 2020

%\cite{Behera:2017xwg}
\bibitem{Behera:2017xwg}
N.~K.~Behera,
%``Constructing probability density function of net-proton multiplicity distributions using Pearson curve method,''
[arXiv:1706.06558 [nucl-ex]].
%3 citations counted in INSPIRE as of 11 Dec 2020

%REF 40
\bibitem{halnpg}
O. Podladchikova, B. Lefebvre, V. Krasnoselskikh, and V. Podladchikov
Nonlinear Processes in Geophysics, European Geosciences Union (EGU) 10, 323 (2003)

%REF 41
%\cite{Adamczyk:2017iwn}
\bibitem{Adamczyk:2017iwn} 
  L.~Adamczyk {\it et al.} [STAR Collaboration],
  \textit{Bulk Properties of the Medium Produced in Relativistic Heavy-Ion Collisions from the Beam Energy Scan Program},
  Phys.\ Rev.\ C {\bf 96}, no. 4, 044904 (2017)
%  doi:10.1103/PhysRevC.96.044904
  [arXiv:1701.07065 [nucl-ex]].
  %%CITATION = doi:10.1103/PhysRevC.96.044904;%%
  %174 citations counted in INSPIRE as of 03 Jan 2020

%REF 42
%\cite{Adcox:2001mf}
\bibitem{Adcox:2001mf} 
  K.~Adcox {\it et al.} [PHENIX Collaboration],
  \textit{Centrality dependence of $pi^{+/-}$, $K^{+/-}$, $p$ and $\overline{p}$ production from $\sqrt{s_{NN}}$ = $130$ GeV Au+Au collisions at RHIC},
  Phys.\ Rev.\ Lett.\  {\bf 88}, 242301 (2002)
 % doi:10.1103/PhysRevLett.88.242301
  [nucl-ex/0112006].
  %%CITATION = doi:10.1103/PhysRevLett.88.242301;%%
  %314 citations counted in INSPIRE as of 03 Jan 2020
 
 %REF 43
  %\cite{Adler:2003cb}
\bibitem{Adler:2003cb} 
  S.~S.~Adler {\it et al.} [PHENIX Collaboration],
  \textit{Identified charged particle spectra and yields in Au+Au collisions at $\sqrt{s_{NN}}$ = 200 GeV},
  Phys.\ Rev.\ C {\bf 69}, 034909 (2004)
%  doi:10.1103/PhysRevC.69.034909
  [nucl-ex/0307022].
  %%CITATION = doi:10.1103/PhysRevC.69.034909;%%
  %874 citations counted in INSPIRE as of 03 Jan 2020
  
  %REF 44
  %\cite{Abelev:2013vea}
\bibitem{Abelev:2013vea} 
  B.~Abelev {\it et al.} [ALICE Collaboration],
  \textit{Centrality dependence of $\pi$, K, p production in Pb-Pb collisions at $\sqrt{s_{NN}}$ = 2.76 TeV},
  Phys.\ Rev.\ C {\bf 88}, 044910 (2013)
%  doi:10.1103/PhysRevC.88.044910
  [arXiv:1303.0737 [hep-ex]].
  %%CITATION = doi:10.1103/PhysRevC.88.044910;%%
  %499 citations counted in INSPIRE as of 03 Jan 2020


%REF 45
\bibitem{elderton}
W. P. Elderton,
\textit{Frequency curves and correlation,} J. Inst. Actuar., William Palin.pp.1-172 (1907)


%REF 46
\bibitem{Lahcene}
B. Lahcene,
\textit{On Pearson families of distributions and its applications}, African Journal of Mathematics and Computer Science Research. Vol. 6(5), pp. 108-117, May 2013. 




\end{thebibliography}
